Finetuning Pre-trained Model with Limited Data for LiDAR-based 3D Object Detection by Bridging Domain Gaps

LiDAR-based 3D object detectors have been largely utilized in various applications, including autonomous vehicles or mobile robots. However, LiDAR-based detectors often fail to adapt well to target domains with different sensor configurations (e.g., types of sensors, spatial resolution, or FOVs) and location shifts. Collecting and annotating datasets in a new setup is commonly required to reduce such gaps, but it is often expensive and time-consuming. Recent studies suggest that pre-trained backbones can be learned in a self-supervised manner with large-scale unlabeled LiDAR frames. However, despite their expressive representations, they remain challenging to generalize well without substantial amounts of data from the target domain. Thus, we propose a novel method, called Domain Adaptive Distill-Tuning (DADT), to adapt a pre-trained model with limited target data (approximately 100 LiDAR frames), retaining its representation power and preventing it from overfitting. Specifically, we use regularizers to align object-level and context-level representations between the pre-trained and finetuned models in a teacher-student architecture. Our experiments with driving benchmarks, i.e., Waymo Open dataset and KITTI, confirm that our method effectively finetunes a pre-trained model, achieving significant gains in accuracy.

==> figs/teaser.tex <==
\begin{figure}[t] 
        \centering
        \includegraphics[width=\linewidth]{assets/teaser_last_last.pdf}
    % \vspace{em}
    \caption{}
    \label{fig:teaser}
    
    
\end{figure}


==> figs/waymo.tex <==
\begin{figure}[t] 
        \centering
        \includegraphics[width=\linewidth]{assets/waymo2.eps}
        \label{fig:waymo}
    \vspace{-4em}
    \caption{Waymo mAP detection performance }
\end{figure}


% \begin{figure}[t]
%     \begin{subfig}
%         \includegraphics[width=\linewidth]{assets/kitti_stats.eps}
%         \label{fig:a}
%     \end{subfig}
%     \begin{subfig}
%         \includegraphics[width=\linewidth]{assets/waymo.eps}
%         \label{fig:b}
%     \end{subfig}
%     \caption{\textbf{KITTI mAP Distribution under Limited Training Samples.} We randomly sampled training frames 5 times from entire training set and measured Car mAP. The performance diverges widely when sampling ratio is relatively small.}\label{fig:kitticar}
% \end{figure}


==> figs/waymo_perform.tex <==
\begin{figure*}[h]
 \begin{minipage}[h]{.7\linewidth}
    \setlength{\tabcolsep}{8pt}
    \renewcommand{\arraystretch}{1.2}
    \centering
     \captionof{table}{Fine-tuning performance on Waymo L1 benchmark}\label{tab:waymo_table}
    \resizebox{\linewidth}{!}{
    \begin{tabular}{ccccccc}
    \toprule
        \multirow{2}{*}{Model} &
        \multirow{2}{*}{Fine-tuning} &
        \multirow{2}{*}{Data Amount(Frames)} & 
        \multicolumn{4}{c}{L1 AP / APH} \\
        \cmidrule{4-7}
         & & & Overall & Vehicle & Pedestrian & Cyclist \\\midrule
    \multirow{8}{*}
    {AD-PT (SECOND)} & Vanilla & 32 & 00.00 / 00.00 & 00.00 / 00.00 & 00.00 / 00.00& 00.00 / 00.00 \\     
        &  \rowcolor{LightBlue}Ours & 32 & 04.44 / 03.81 & 10.91 / 10.66 & 01.66 / 01.15 & 00.77 / 00.71 \\ 
        & Vanilla & 64 & 02.75 / 02.71 & 05.98 / 05.90 & 00.01 / 00.00 & 02.26 / 02.23 \\  
        &  \rowcolor{LightBlue} Ours & 64 & 23.73 / 21.48 & 25.74 / 25.29 & 17.05 / 11.64 & 28.39 / 27.51  \\
        & Vanilla & 95 & 15.02 / 14.11 & 14.76 / 14.51 & 07.22 / 05.21& 23.07 / 22.62 \\ 
        &  \rowcolor{LightBlue} Ours & 95 & 33.77 / 30.55 & 37.65 / 37.03 & 26.33 / 18.30 & 37.34 / 36.32 \\ 
        & Vanilla & 127 & 33.07 / 30.34 & 34.96 / 34.35 & 27.26 / 20.52 & 37.00 / 36.16 \\ 
        &  \rowcolor{LightBlue} Ours & 127 & 40.22 / 36.75 & 46.48 / 45.71 & 33.33 / 24.67 & 40.85 / 39.89 \\ 
         
    \bottomrule 
    \end{tabular}}
   
    \end{minipage}
  \begin{minipage}[h]{.3\linewidth}
    \centering
   
    \includegraphics[width=\linewidth]{assets/waymo2.eps}
    \captionof{figure}{Waymo AP Benchmark}\label{fig:waymo_mAP}
  \end{minipage}
 
\end{figure*}





==> tables/DA.tex <==
{
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{1} 
\begin{table}[t]
	\begin{center}
        \caption{Domain Adaptation Performance}
    	\resizebox{.85\linewidth}{!}{%
    	\begin{tabular} {@{}lcccc@{}} \toprule
            \multirow{2}{*}{Waymo \xrightarrow{} KITTI}  & \multicolumn{3}{c}{$AP_{3D}$} \\\cmidrule{2-4}
              & Easy & Moderate & Hard \\ \midrule
            Direct Transfer  &78.05 & 63.67 & 59.35\\
            Vanilla  &81.19 & 64.02 & 59.54\\
            Ours (only KITTI)  &82.48 & 65.27 & \textbf{60.95}\\
            \midrule
            \textbf{Ours (DADT)}  & \textbf{83.84} & \textbf{66.07} &60.89 \\
            \bottomrule
            \end{tabular}}
        \label{tab:DA}
     \end{center}\vspace{-2em}
\end{table}
}

==> tables/dataset_density.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
{
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{1}
\begin{table}[t]
    \centering
    \caption{Dataset details.}
    \resizebox{\linewidth}{!}{%
    \begin{tabular}{lcccc}
        \toprule
        Dataset & VFOV & \# of Beams & \# of Avg. Points & Location \\ \midrule
        ONCE~\cite{ONCE} & [-25$^{\circ}$, -15$^{\circ}$] &  40 & 64,981 & China\\ 
        Waymo~\cite{waymo} &[-17.6$^{\circ}$, -2.4$^{\circ}$] & 64 & 160,887 & USA\\ 
        KITTI~\cite{kitti} & [-25$^{\circ}$, -15$^{\circ}$] & 64 & 119,748 & Germany\\
        \bottomrule
    \end{tabular}%
}
% \vspace{-3em}
\label{tab:beam}
\end{table}
}
%Pseudo Waymo & 32 & 89212 \\ 
%Pseudo KITTI & 32 & 59946 \\ \bottomrule

==> tables/kitti.tex <==
\setlength{\tabcolsep}{8pt}
\renewcommand{\arraystretch}{1.2}
\begin{table*}[h]
    \centering
    \caption{\textbf{3D Detection Accuracy Comparison on KITTI Dataset.} We report scores in terms of 3D Average Precision (AP), with the IoU threshold set to 0.7 for Cars and 0.5 for Pedestrians and Cyclists.}
    \label{tab:kitti}
    \resizebox{.4\linewidth}{!}{
    
    \begin{tabular}{lccc}
    \toprule
        \multirow{2}{*}{Finetuning} & \multirow{2}{*}{\# of Data} & \multicolumn{2}{c}{mAP (Mod.)}\\ \cmidrule{3-4}
        && SECOND & PV-RCNN++\\\midrule
        Vanilla & 1\% & 16.76 & 15.85\\    
        \rowcolor{LightGrey} Ours & 1\% & 21.66 & 20.21\\ 
        \rowcolor{LightGrey} & & (\red{00.00$\uparrow$}) & (\red{00.00$\uparrow$})\\ \midrule
        Vanilla & 2\% & 29.60 & 40.94 \\  
        \rowcolor{LightGrey}  Ours & 2\% & 31.28 & 44.49 \\
        \rowcolor{LightGrey} & & (\red{00.00$\uparrow$}) & (\red{00.00$\uparrow$})\\ \midrule
        Vanilla & 3\% & 38.91 & 49.53 \\ 
        \rowcolor{LightGrey}  Ours & 3\% & 42.24 & 54.73\\ 
        \rowcolor{LightGrey} & & (\red{00.00$\uparrow$}) & (\red{00.00$\uparrow$})\\
    \bottomrule 
    \end{tabular}}
    
\end{table*}


% \setlength{\tabcolsep}{8pt}
% \renewcommand{\arraystretch}{1.2}
% \begin{table*}[h]
%     \centering
%     \caption{Fine-tuning performance on KITTI benchmark ($AP_{3D}$).
%     The evaluation metric is Average Precision (AP) with IoU threshold 0.7 for Car and 0.5 for Pedestrian \& Cyclist.}
%     \label{tab:kitti}
%     \resizebox{\linewidth}{!}{
    
%     \begin{tabular}{l|c|c|c|ccc|ccc|ccc|}
%     \toprule
%     \multirow{2}{*}{Model} & \multirow{2}{*}{Fine-tuning} & \multirow{2}{*}{Data Amount} & \multirow{2}{*}{mAP (Mod.)} &  \multicolumn{3}{c|}{Car} & \multicolumn{3}{c|}{Pedestrian} & \multicolumn{3}{c|}{Cyclist}\\
%     \cmidrule{5-13}
%     &&&&Easy&Mod.&Hard&Easy&Mod.&Hard&Easy&Mod.&Hard\\
%     \midrule \midrule
%     \multirow{8}{*}
%     {AD-PT (SECOND)} & Vanilla & 1\% & 16.76&  24.59 & 20.16 &  \multicolumn{1}{c|}{20.08} & 9.38 & 8.37 &  \multicolumn{1}{c|}{8.04}& 35.28 & 21.76 & \multicolumn{1}{c|}{20.52}\\     
%         &  \rowcolor{LightBlue} Ours & 1\% & 21.66 & 35.39 & 28.21& \multicolumn{1}{c|}{26.94}& 11.51 & 10.21& \multicolumn{1}{c|}{9.60}& 43.17 & 26.56& \multicolumn{1}{c|}{24.78} \\ 
%         & Vanilla & 2\% & 29.60 & 46.90 & 36.94& \multicolumn{1}{c|}{35.19} & 26.08 & 22.63& \multicolumn{1}{c|}{21.06}& 45.84 & 29.23& \multicolumn{1}{c|}{27.90}\\  
%         & \rowcolor{LightBlue}  Ours & 2\% & 31.28 & 47.56 & 38.26 & \multicolumn{1}{c|}{35.79} & 27.52 & 23.33& \multicolumn{1}{c|}{21.76}& 50.34 & 32.24&\multicolumn{1}{c|}{31.11}\\
%         & Vanilla & 3\% & 38.91 & 64.31 & 50.54& \multicolumn{1}{c|}{47.66}& 38.34 & 31.80& \multicolumn{1}{c|}{29.69}& 53.37 & 34.39& \multicolumn{1}{c|}{32.96} \\ 
%         & \rowcolor{LightBlue}  Ours & 3\% & 42.24 & 65.78 & 52.63& \multicolumn{1}{c|}{49.55}& 41.59 & 35.26& \multicolumn{1}{c|}{32.77}& 60.04 & 38.83& \multicolumn{1}{c|}{37.39} \\ 
%         % & Vanilla & 4\% & 51.53 & 80.83 & 65.51& \multicolumn{1}{c|}{61.42}& 44.63 & 38.76& \multicolumn{1}{c|}{36.30}& 72.09 & 50.32& \multicolumn{1}{c|}{47.79} \\ 
%         % & \rowcolor{LightBlue}  Ours & 4\% & 51.30 & 79.55 & 65.94& \multicolumn{1}{c|}{62.14}& 45.30 & 38.72& \multicolumn{1}{c|}{36.32}& 71.88 & 49.24& \multicolumn{1}{c|}{46.79} \\ 
%     \midrule
%     \multirow{8}{*}
%     {AD-PT (PV-RCNN++)} & Vanilla & 1\% & 15.85 & 26.99 & 19.89& \multicolumn{1}{c|}{18.22}& 18.08 & 16.61& \multicolumn{1}{c|}{14.95}& 16.46 & 11.04 & \multicolumn{1}{c|}{10.41}\\     
%         & \rowcolor{LightBlue} Ours & 1\% & 20.21 & 31.98 & 23.60& \multicolumn{1}{c|}{21.42}& 24.37 & 21.50& \multicolumn{1}{c|}{19.16}& 22.3 & 15.53 & \multicolumn{1}{c|}{14.61} \\ 
%         & Vanilla & 2\% & 40.94 & 69.32 & 51.02& \multicolumn{1}{c|}{47.33} & 48.97 & 42.63& \multicolumn{1}{c|}{38.19}& 42.62 & 29.16 & \multicolumn{1}{c|}{27.76}\\  
%         & \rowcolor{LightBlue}  Ours & 2\% & 44.49 & 69.72 & 52.08 & \multicolumn{1}{c|}{47.71} & 52.77 & 45.87& \multicolumn{1}{c|}{41.36}& 52.91 & 35.50&\multicolumn{1}{c|}{34.15}\\
%         & Vanilla & 3\% & 49.53 & 81.19 & 64.02& \multicolumn{1}{c|}{59.54}& 52.13 & 43.89& \multicolumn{1}{c|}{38.81}& 55.42 & 40.68& \multicolumn{1}{c|}{38.82} \\ 
%         &  \rowcolor{LightBlue} Ours & 3\% & 54.73 & 82.48 & 65.27& \multicolumn{1}{c|}{60.95}& 57.60 & 49.67& \multicolumn{1}{c|}{44.31}& 68.97 & 49.24& \multicolumn{1}{c|}{46.89} \\ 
%         % & Vanilla & 4\% & 62.73 & 88.59 & 72.30& \multicolumn{1}{c|}{69.48}& 62.73 & 55.04 & \multicolumn{1}{c|}{49.87}& 81.44 & 60.86& \multicolumn{1}{c|}{57.51} \\ 
%         % & \rowcolor{LightBlue}  Ours & 4\% & 62.98 & 88.95 & 74.30& \multicolumn{1}{c|}{70.29}& 62.27 & 54.36& \multicolumn{1}{c|}{48.98}& 81.13 & 60.28& \multicolumn{1}{c|}{56.65} \\ 
%     \bottomrule 
%     \end{tabular}}
    
% \end{table*}

==> tables/teacher.tex <==
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{1} 
\begin{table}[t]
	\begin{center}
        
    	\resizebox{.85\linewidth}{!}{%
    	\begin{tabular} {@{}ccccc@{}} \toprule
            \multirow{2}{*}{Teacher Beam Numbers}  & \multicolumn{3}{c}{$AP_{3D}$} \\\cmidrule{2-4}
              & Easy & Moderate & Hard \\ \midrule
            64  &- & - & -\\
            32\^  &- & - & -\\ 
            \midrule
            \textbf{32}  & - & -&- \\
            
            \bottomrule
            \end{tabular}}
        \caption{Ablation on different types of teacher datasets.}
        \label{tab:teacher}
     \end{center}\vspace{-2em}
\end{table}

==> tables/waymo.tex <==

% \setlength{\tabcolsep}{8pt}
% \renewcommand{\arraystretch}{1.2}
% \begin{table*}[h]
%     \centering
%     \resizebox{\linewidth}{!}{
    
%     \begin{tabular}{ccccccc}
%     \toprule
%         \multirow{2}{*}{Model} &
%         \multirow{2}{*}{Fine-tuning} &
%         \multirow{2}{*}{Data Amount(Frames)} & 
%         \multicolumn{4}{c}{L1 AP / APH} \\
%         \cmidrule{4-7}
%          & & & Overall & Vehicle & Pedestrian & Cyclist \\\midrule
%     \multirow{10}{*}
%     {AD-PT (SECOND)} & Vanilla & 32 & 00.00 / 00.00 & 00.00 / 00.00 & 00.00 / 00.00& 00.00 / 00.00 \\     
%         &  \rowcolor{LightBlue}Ours & 32 & 04.44 / 03.81 & 10.91 / 10.66 & 01.66 / 01.15 & 00.77 / 00.71 \\ 
%         & Vanilla & 64 & 02.75 / 02.71 & 05.98 / 05.90 & 00.01 / 00.00 & 02.26 / 02.23 \\  
%         &  \rowcolor{LightBlue} Ours & 64 & 23.73 / 21.48 & 25.74 / 25.29 & 17.05 / 11.64 & 28.39 / 27.51  \\
%         & Vanilla & 96 & 15.02 / 14.11 & 14.76 / 14.51 & 07.22 / 05.21& 23.07 / 22.62 \\ 
%         &  \rowcolor{LightBlue} Ours & 96 & 33.77 / 30.55 & 37.65 / 37.03 & 26.33 / 18.30 & 37.34 / 36.32 \\ 
%         & Vanilla & 128 & 33.07 / 30.34 & 34.96 / 34.35 & 27.26 / 20.52 & 37.00 / 36.16 \\ 
%         &  \rowcolor{LightBlue} Ours & 128 & 40.22 / 36.75 & 46.48 / 45.71 & 33.33 / 24.67 & 40.85 / 39.89 \\ 
         
%     \midrule
%     \multirow{8}{*}
%     {AD-PT (PV-RCNN++)} & Vanilla & 32 & - & - & -& - \\     
%         &  \rowcolor{LightBlue} Ours & 32 & - & - & -& - \\
%         & Vanilla & 64 & - & - & -& - \\ 
%         & \rowcolor{LightBlue}  Ours & 64 & - & - & -& - \\
%         & Vanilla & 96 & 35.30 / 32.79 & 41.58 / 40.88 & 31.55 / 25.91 & 32.78 / 31.58 \\ 
%         &  \rowcolor{LightBlue} Ours & 96 & 36.49 / 33.89 & 42.82 / 42.17 & 33.54 / 27.35 & 33.11 / 32.14 \\
%         & Vanilla & 128 & 48.78 / 45.57 & 54.41 / 53.72 & 46.85 / 38.99 & 45.09 / 44.00 \\ 
%         &  \rowcolor{LightBlue} Ours & 128 & 48.28 / 45.16 & 53.42 / 52.74 & 45.62 / 38.05 & 45.80 / 44.71 \\
        
%     \bottomrule 
%     \end{tabular}}
%     \caption{Fine-tuning performance on Waymo L1 benchmark}
%     \label{tab:waymo}
% \end{table*}



% \setlength{\tabcolsep}{8pt}
% \renewcommand{\arraystretch}{1.1}
% \begin{table*}[h]
%     \centering
%     \resizebox{\linewidth}{!}{ 
%     \begin{tabular}{ccccccc}
%     \toprule
%         \multirow{2}{*}{Model} &
%         \multirow{2}{*}{Fine-tuning} &
%         \multirow{2}{*}{Data Amount(Frames)} & 
%         \multicolumn{4}{c}{L1 AP / APH} \\
%         \cmidrule{4-7}
%          & & & Overall & Vehicle & Pedestrian & Cyclist \\\midrule
%     \multirow{8}{*}
%     {AD-PT (SECOND)} & Vanilla & 32 & 00.00 / 00.00 & 00.00 / 00.00 & 00.00 / 00.00& 00.00 / 00.00 \\     
%         &  \rowcolor{LightBlue}Ours & 32 & 04.44 / 03.81 & 10.91 / 10.66 & 01.66 / 01.15 & 00.77 / 00.71 \\ 
%         & Vanilla & 64 & 02.75 / 02.71 & 05.98 / 05.90 & 00.01 / 00.00 & 02.26 / 02.23 \\  
%         &  \rowcolor{LightBlue} Ours & 64 & 23.73 / 21.48 & 25.74 / 25.29 & 17.05 / 11.64 & 28.39 / 27.51  \\
%         & Vanilla & 96 & 15.02 / 14.11 & 14.76 / 14.51 & 07.22 / 05.21& 23.07 / 22.62 \\ 
%         &  \rowcolor{LightBlue} Ours & 96 & 33.77 / 30.55 & 37.65 / 37.03 & 26.33 / 18.30 & 37.34 / 36.32 \\ 
%         & Vanilla & 128 & 33.07 / 30.34 & 34.96 / 34.35 & 27.26 / 20.52 & 37.00 / 36.16 \\ 
%         &  \rowcolor{LightBlue} Ours & 128 & 40.22 / 36.75 & 46.48 / 45.71 & 33.33 / 24.67 & 40.85 / 39.89 \\ 
%     \bottomrule 
%     \end{tabular}}
%     \caption{Fine-tuning performance on Waymo L1 benchmark}
%     \label{tab:waymo}
% \end{table*}


\setlength{\tabcolsep}{8pt}
\renewcommand{\arraystretch}{1.1}
\begin{table*}[h]
    \centering
    \caption{\textbf{3D Detection Accuracy Comparison with Limited Data.} We compare the detection performance of finetuned models with limited data, from 32 to 128, in terms of the two primary metrics of Waymo Open Dataset: AP and APH. Note that we use the whole validation set to measure scores.}
    \label{tab:waymo}
    \resizebox{.7\linewidth}{!}{ 
    \begin{tabular}{lccccc}
    \toprule
        \multirow{2}{*}{Finetuning} &
        \multirow{2}{*}{\# of Data} & 
        \multicolumn{4}{c}{AP / APH} \\
        \cmidrule{3-6}
        & & Overall & Vehicle & Pedestrian & Cyclist \\\midrule
        Vanilla & 32 & 00.00 / 00.00 & 00.00 / 00.00 & 00.00 / 00.00& 00.00 / 00.00 \\     
        \rowcolor{LightGrey} Ours & 32 & 04.44 / 03.81 & 10.91 / 10.66 & 01.66 / 01.15 & 00.77 / 00.71 \\
        \rowcolor{LightGrey} &  & (\red{4.44$\uparrow$ / 3.81$\uparrow$})  & (\red{10.91$\uparrow$ / 10.66$\uparrow$}) & (\red{1.66$\uparrow$ / 1.15$\uparrow$}) & (\red{0.77$\uparrow$ / 0.71$\uparrow$})\\
        \midrule  
        Vanilla & 64 & 02.75 / 02.71 & 05.98 / 05.90 & 00.01 / 00.00 & 02.26 / 02.23 \\ 
        \rowcolor{LightGrey} Ours & 64 & 23.73 / 21.48 & 25.74 / 25.29 & 17.05 / 11.64 & 28.39 / 27.51  \\
        \rowcolor{LightGrey} &  & (\red{4.44$\uparrow$ / 3.81$\uparrow$})  & (\red{10.91$\uparrow$ / 10.66$\uparrow$}) & (\red{1.66$\uparrow$ / 1.15$\uparrow$}) & (\red{0.77$\uparrow$ / 0.71$\uparrow$})\\\midrule 
        Vanilla & 96 & 15.02 / 14.11 & 14.76 / 14.51 & 07.22 / 05.21& 23.07 / 22.62 \\ 
        \rowcolor{LightGrey} Ours & 96 & 33.77 / 30.55 & 37.65 / 37.03 & 26.33 / 18.30 & 37.34 / 36.32 \\
        \rowcolor{LightGrey} &  & (\red{4.44$\uparrow$ / 3.81$\uparrow$})  & (\red{10.91$\uparrow$ / 10.66$\uparrow$}) & (\red{1.66$\uparrow$ / 1.15$\uparrow$}) & (\red{0.77$\uparrow$ / 0.71$\uparrow$})\\\midrule  
        Vanilla & 128 & 33.07 / 30.34 & 34.96 / 34.35 & 27.26 / 20.52 & 37.00 / 36.16 \\ 
        \rowcolor{LightGrey} Ours & 128 & 40.22 / 36.75 & 46.48 / 45.71 & 33.33 / 24.67 & 40.85 / 39.89 \\\rowcolor{LightGrey} &  & (\red{4.44$\uparrow$ / 3.81$\uparrow$})  & (\red{10.91$\uparrow$ / 10.66$\uparrow$}) & (\red{1.66$\uparrow$ / 1.15$\uparrow$}) & (\red{0.77$\uparrow$ / 0.71$\uparrow$})\\
    \bottomrule 
    \end{tabular}}
\end{table*}
